A Method for Distributed Transactive Control in Power Systems based on the Projected Consensus Algorithm

The shift of power systems toward a smarter grid has brought devices such as distributed generators and smart loads with an increase of the operational challenges for the system operator. These challenges are related to the real-time implementation as well as control and stability issues. We present a distributed transactive control strategy, based on the projected consensus algorithm, to operate the distributed energy resources and smart loads of a power system toward optimal social welfare. We consider two types of agents: Generators, and smart loads. Each agent iteratively optimizes its local utility function based on local information obtained from its neighbors and global information obtained through the network of agents. We show convergence analysis and numerical results for the proposed method.

==> Images/graph.tex <==
% Declare layers
\pgfdeclarelayer{background}
\pgfsetlayers{background,main}

%% Adjacency matrix of graph
%% \  a  b  c  d  e  f  g
%% a  x  7     5
%% b  7  x  8  9  7
%% c     8  x     5
%% d  5  9     x 15  6
%% e     7  5 15  x  8  9
%% f           6  8  x 11
%% g              9  11 x

\tikzstyle{vertex}=[circle,fill=black!25,minimum size=20pt,inner sep=0pt]
\tikzstyle{selected vertex} = [vertex, fill=gray!24]
\tikzstyle{edge} = [draw,thick,-]
\tikzstyle{weight} = [font=\small]
\tikzstyle{selected edge} = [draw,line width=5pt,-,fill=gray!50,fill opacity=0.6]
\tikzstyle{tree edge} = [draw,line width=5pt,-,blue!50]



\begin{tikzpicture}[scale=2.2, auto,swap]
    % Draw a 7,11 network
    % First we draw the vertices
    \foreach \pos/\name in {{(0,1)/a}, {(2,1)/b}, {(4,1)/c},
                            {(0,-1)/d}, {(3,0)/e}, {(2,-1)/f}, {(4,-1)/g}}
        \node[vertex] (\name) at \pos {$\name$};
    % Connect vertices with edges and draw weights
    \foreach \source/ \dest  in {b/a, c/b,d/a,d/b,e/b, e/c,f/d,f/e,g/e,g/f}
        \path[edge] (\source) --  (\dest);
      % Colored the vertices
    \foreach \pos/\name in {{(0,1)/a}, {(2,1)/b}, {(3,0)/e}, {(4,-1)/g}}
        \node[selected vertex] (\name) at \pos {$\name$};
        
    % Colored vertices with edges and draw path
    \foreach \source/ \dest in {b/a, e/b,g/e}
        \path[selected edge] (\source) -- (\dest);
        
    % Connect vertices with edges and draw weights
    \foreach \source/ \dest  in { d/a,d/b, e/c,f/d,f/e,g/f}
        \path[tree edge] (\source) --  (\dest);        
  
  \end{tikzpicture}
